VDPP: Video Depth Post-Processing for Speed and Scalability

Video depth estimation is essential for providing 3D scene structure in applications ranging from autonomous driving to mixed reality. Current end-to-end video depth models have established state-of-the-art performance. Although current end-to-end (E2E) models have achieved state-of-the-art performance, they function as tightly coupled systems that suffer from a significant adaptation lag whenever superior single-image depth estimators are released. To mitigate this issue, post-processing methods such as NVDS offer a modular plug-and-play alternative to incorporate any evolving image depth model without retraining. However, existing post-processing methods still struggle to match the efficiency and practicality of E2E systems due to limited speed, accuracy, and RGB reliance. In this work, we revitalize the role of post-processing by proposing VDPP (Video Depth Post-Processing), a framework that improves the speed and accuracy of post-processing methods for video depth estimation. By shifting the paradigm from computationally expensive scene reconstruction to targeted geometric refinement, VDPP operates purely on geometric refinements in low-resolution space. This design achieves exceptional speed (>43.5 FPS on NVIDIA Jetson Orin Nano) while matching the temporal coherence of E2E systems, with dense residual learning driving geometric representations rather than full reconstructions. Furthermore, our VDPP's RGB-free architecture ensures true scalability, enabling immediate integration with any evolving image depth model. Our results demonstrate that VDPP provides a superior balance of speed, accuracy, and memory efficiency, making it the most practical solution for real-time edge deployment. Our project page is at https://github.com/injun-baek/VDPP

==> sec/0_abstract_yr.tex <==
% E2E/I2D의 한계 지적 → Post-processing의 당위성 → VDPP의 독보적 성능
\begin{abstract}
Video depth estimation \yr{is essential for providing 3D scene structure in applications ranging from autonomous driving to mixed reality.} % provides 3D scene information from standard 2D video for applications in VR, AR, autonomous driving, collision detection, etc.
\yr{While c}urrent end-to-end (E2E) models have achieved state-of-the-art performance, they function as tightly coupled systems \yr{that suffer from} a significant adaptation lag whenever superior single-image depth estimators are released.
\yr{To mitigate this issue, post-processing methods have emerged as a modular plug-and-play alternative that can theoretically incorporate any evolving image-level depth model without retraining.
However, existing post-processing methods still fail to match the efficiency and practicality of E2E systems due to their heavy reliance on RGB data and high computational latency.}
\yr{In this work, we revitalize the role of post-processing by proposing} \textbf{VDPP (Video Depth Post-Processing)}, a framework that improves the speed and accuracy of post-processing methods for video depth estimation.
\yr{By shifting the paradigm from computationally expensive scene reconstruction to targeted geometric refinement, VDPP operates purely on geometric representations in low-resolution space.
By learning dense residual predictions rather than full reconstructions,}
% By operating on geometric representations in low-resolution space and learning only dense residual prediction rather than full reconstructions, 
our method achieves exceptional speed ($>43.5$ FPS on NVIDIA Jetson Orin Nano) \yr{while matching the temporal coherence of heavy E2E systems}. % This speed does not compromise accuracy. 
\yr{Furthermore, VDPP’s RGB-free architecture ensures true scalability, enabling immediate integration with any evolving image depth model or direct refinement of noisy depth sensors.} % In addition, VDPP operates purely on depth information without any RGB dependency, achieving scalability.
%This enables true plug-and-play compatibility with any image depth model, effectively reducing the memory requirements for real-time deployment. 
\yr{Our results demonstrate that VDPP provides a superior balance of speed, accuracy, and memory efficiency, making it the most practical solution for real-time edge deployment.}
\end{abstract}


==> sec/1_intro.tex <==
\section{Introduction}

% \dw{문제인식:VDA같은 End to End가 SOTA 인정. 하지만 End to End는 monolithic arch이기 때문에 Image Depth 새롭게 출시되어도 video에 적용하기에는 시간텀이 있어. 그럴때 post-processing이 필요한데 그나마 최신 기술 NVDS가 속도과 정확도 측면에서 많이 부족하다. 그걸 우리가 개선해주겠다고 겸손하게 접근 필요 (나머지 장점들은 그냥 덤덤하게 실험에서 풀고 결론에 덧붙이지 뭐)}

%중요한 연구 배경
Video depth estimation, the task of inferring 3D scene structure from 2D video sequences, is important as a cornerstone technology for a variety of modern applications such as autonomous driving, robotics, and mixed reality. Driven by the critical need, monolithic end-to-end (E2) models such as Video Depth Anything (VDA)~\cite{vda} have established the current state-of-the-art, delivering exceptional coherence and spatial accuracy. 


However, these models are typically designed as tightly coupled systems, leading to lag in the latest adaptation. Whenever the latest single-image depth estimator is released, it cannot be easily integrated into existing end-to-end frameworks without full-scale retraining. Moreover, these massive all-in-one systems are often too heavy for the limited memory of edge devices. 
While modular post-processing methods like NVDS~\cite{nvds} offer a plug-and-play alternative, they have yet to match the efficiency of end-to-end systems. Existing post-processing frameworks often suffer from taking orders of magnitude long inference and reliance on RGB data, which are critical bottlenecks for real-time applications.

In this work, we revitalize the role of post-processing in video depth estimation. We demonstrate that post-processing can achieve not only competitive accuracy, but also superior speed and scalability. By moving away from monolithic architectures, our approach allows for the immediate evaluation and integration of the latest image-depth models in video streams. Furthermore, by avoiding computational overhead, our framework can be deployed on resource-constrained devices where memory is strictly limited. 
we propose a shift in perspective: rather than reconstructing the full 3D world by analyzing all the complex color context in an RGB video, as a process that makes existing post-processing models like NVDS~\cite{nvds, nvdsplus} computationally expensive, we argue for efficiently geometric refining and restoring. Our method starts with a simple assumption. The per-frame depth maps give us an unstable but already good 3D structure. This reframes the task from a scene reconstruction problem into a much more manageable structure correction problem. We do not need to rebuild the world from color. We only need to fix the unstable elements using a few powerful geometric clues. Our work not only reduces the barrier for deploying rapid video depth in practical applications but also contributes a new, scalable paradigm for leveraging geometry-only information to ensure temporal stability.


As shown in Table~\ref{tab:comparison}, current video depth solutions often involve trade-offs in practical deployment. High-performance end-to-end models such as VDA-L~\cite{vda} establish a benchmark for temporal coherence, but their monolithic designs are typically too computationally intensive for real-time edge use. Although modular post-processing methods like NVDS~\cite{nvds} aim to bridge this gap, they often suffer from latency and reliance on RGB data, failing to reach the efficiency required for embedded applications. In contrast, state-of-the-art single-image estimators such as DAv2~\cite{depthanythingv2} provide spatial accuracy and speed, but lack the inherent temporal coherence for stable video streams.


% \begin{table}[t]
% \centering
% \caption{\textbf{Comparison of video depth methods.} VDPP uniquely satisfies all requirements of speed, accuracy, and scalability.}
% \label{tab:comparison}
% \small
% \setlength{\tabcolsep}{4pt} % 열 간격 줄이기
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l|ccccc}
% \toprule
% \textbf{Method} & \textbf{Speed} & \textbf{Spatial \&} & \textbf{Plug \&} & \textbf{Depth} & \textbf{Light-} \\
%  & \textbf{($>30$ FPS)} & \textbf{Temporal} & \textbf{Play} & \textbf{Only} & \textbf{weight} \\
% \midrule
% VDA-S & \checkmark & $\triangle$ & $\times$ & $\times$ & $\times$ \\
% VDA-L & $\times$ & \checkmark & $\times$ & $\times$ & $\times$ \\
% NVDS & $\times$ & $\triangle$ & \checkmark & $\times$ & $\times$ \\
% DAv2 & \checkmark & $\times$ & $\times$ & $\times$ & \checkmark \\
% \rowcolor{green!15}
% \textbf{Ours (VDPP)} & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
% \bottomrule
% \end{tabular}}
% \raggedright
% \footnotesize
% \textbf* Light-weight capability is defined by the ability to run successfully on resource-constrained platforms, specifically tested against the NVIDIA Jetson Orin Nano (8GB) without encountering Out-of-Memory errors.
% \vspace{-5mm}
% \end{table}

\begin{table}[t]
\centering
\caption{\textbf{Comparison of video depth estimation paradigms.} VDPP provides a balanced profile for practical deployment, achieving SOTA-level coherence within a modular and efficient post-processing framework.}
\label{tab:comparison}
\small
\setlength{\tabcolsep}{5pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|l|ccccc}
\toprule
\textbf{Category} & \textbf{Method} & \textbf{Speed} & \textbf{Temporal} & \textbf{Plug \&} & \textbf{Depth} & \textbf{Light-} \\
 & & \textbf{($>30$ FPS)} & \textbf{Coherence} & \textbf{Play} & \textbf{Only} & \textbf{weight} \\
\midrule
\multirow{2}{*}{End-to-End} & VDA-S~\cite{vda} & \checkmark & $\triangle$ & $\times$ & $\times$ & $\times$ \\
 & VDA-L~\cite{vda} & $\times$ & \checkmark & $\times$ & $\times$ & $\times$ \\
\midrule
\multirow{2}{*}{Post-Processing} & NVDS~\cite{nvds} & $\times$ & $\times$ & \checkmark & $\times$ & $\times$ \\
% \rowcolor{green!15}
 & \textbf{VDPP (Ours)} & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
\bottomrule
\end{tabular}}
\raggedright
\footnotesize
% \vspace{1mm}

% * DAv2~\cite{depthanythingv2} serves as the image depth estimation for post-processing.\\
%   Although it achieves exceptional spatial accuracy and speed ($>30$ FPS), it does not satisfy the temporal coherence requirements for stable video.\\
* Lightweight capability is verified on the NVIDIA Jetson Orin Nano (8GB) without Out-of-Memory errors.
\vspace{-4mm}
\end{table}

%우린 이런 방법으로 설계했다.
We propose\textbf{ VDPP (Video Depth Post-Processing)}, a framework that formulates video depth stabilization as a targeted geometric correction problem. By precisely refining unstable per-frame depth sequences, our approach overcomes the efficiency and accuracy bottlenecks of previous post-processing methods. This allows VDPP to bring robust coherence to real-time embedded applications without losing the inherent flexibility of a modular architecture. Figure~\ref{fig:teaser} provides a qualitative and quantitative overview of our results. The left side displays the qualitative refinement achieved by VDPP, while the right side presents a quantitative comparison graph based on the Sintel dataset~\cite{sintel} at a resolution of $384 \times 384$. The detailed numerical tables supporting this graph are provided in Appendix C.

\begin{itemize}
\item \textbf{Decoupled and Scalable Paradigm:} We propose an RGB-free, modular framework that revitalizes the role of post-processing. By eliminating the dependency on color context, we resolve the adaptation lag of monolithic models, enabling the immediate integration of any evolving image-depth backbone or depth-only sensors (e.g., LiDAR) into stable video streams.

\item \textbf{Embedded Efficiency and Real-time Deployment:} Designed specifically for resource-constrained environments, VDPP overcomes the latency bottlenecks of previous post-processing methods. We demonstrate that our framework achieves remarkable efficiency, reaching $> 43.5$ FPS on an NVIDIA Jetson Orin Nano with minimal memory footprint, making high-quality video depth viable for real-time edge applications.

\item \textbf{Geometric Refinement with Residual Learning:} We introduce a dual-component design (Depth + Normals) with downsampling combined with residual learning in error space. This technical shift focuses the network on targeted geometric correction rather than redundant scene reconstruction, allowing a lightweight architecture to match the temporal coherence of heavy end-to-end systems.

\end{itemize}


% \dw{전개 방식이나 마지막 노벨티 강조하는 부분 변경 원하시면 변경하시고 메모 남겨주세요}
% \inj{우리가 빠르고 경량이라는게 메인 contribution 이기 때문에, 이것을 더 먼저 나열하는게 좋을것같습니다.}
% \dw{contribution item 순서 변경 완료}

% In fields such as autonomous driving, robotics, virtual reality, and augmented reality, the ability to perceive and understand geometric depth information is not only useful but also essential for safe and immersive human-machine interaction in the real world. A rapid and stable stream of depth information allows machines to navigate complex environments, enables virtual objects to seamlessly integrate into real space, and provides critical information for collision avoidance. 

% Despite its importance, the field currently faces a dilemma that forces practitioners to sacrifice at least one of three essential properties: speed, accuracy, and scalability. No existing approach successfully achieves all three simultaneously, leaving a critical gap in practical deployment. \textbf{Problem 1: Fast but Inconsistent}. The fastest approach is undoubtedly applying state-of-the-art single-image depth models like Depth Anything V2~(DAv2)~\cite{depthanythingv2} on a per-frame basis, achieving the fastest inference time. However, the complete lack of temporal context results in severe flicker artifacts, rendering the output unusable for video despite high per-frame quality. Even though dedicated video models optimized for speed, like Video Depth Anything Small (VDA-S)~\cite{vda}, show some progress, they still sacrifice accuracy and scalability. VDPP ultimately delivers better accuracy and scalability.
% \textbf{Problem 2: Accurate but Slow}. For the highest accuracy and temporal coherence, end-to-end models Video Depth Anything Large (VDA-L)~\cite{vda} currently represent the state-of-the-art. However, this accuracy comes at a significant cost. Its computationally intensive spatio-temporal attention processing on RGB input video results in very slow inference speeds, struggling to exceed 20 FPS on a NVIDIA RTX A6000 GPU, making it impractical for real-time applications.
% \textbf{Problem 3: Scalable but Limited}. Post-processing methods such as Neural Video Depth Stabilizer~(NVDS)~\cite{nvds, nvdsplus} introduced the conceptually appealing plug-and-play paradigm, aiming to leverage the advancements in single-image depth estimation. This approach offers the potential advantage of incorporating newer, more powerful image depth models as they emerge. However, NVDS requires a refinement stage that takes approximately 30 times longer than the image depth estimation like DAv2-B~\cite{depthanythingv2}, and its simple global correction mechanism fails to achieve spatial and temporal accuracy. More fundamentally, both post-processing methods like NVDS and end-to-end models like VDA share a limitation: they rely on RGB input for their processing. This inherent RGB dependency renders them incompatible with increasingly important depth-only data sources such as LiDAR or ToF sensors, severely limiting their real-world applicability and scalability.

%우린 문제를 이런 아이디어로 접근한다.
%In this work, we argue for a fundamental shift in perspective to resolve this trade-off. Models like VDA try to solve a very hard problem. They build a 3D space by analyzing all the complex color context in an RGB video. We think this approach is often unnecessarily complex. We believe a smarter solution is to intelligently and rapidly restore an already good result, not to reconstruct the entire world.

%문제배경은 E2E의 monolithic structure로 인한 image depth와의 gap, 리소스 제한 상황에서의 챌린지. 하지만 post-processing은 e2e보다 성능과 속도가 떨어져서 외면받고 쓸수없는 상황인것이다.

==> sec/1_intro_yr.tex <==
\section{Introduction}

% \dw{문제인식:VDA같은 End to End가 SOTA 인정. 하지만 End to End는 monolithic arch이기 때문에 Image Depth 새롭게 출시되어도 video에 적용하기에는 시간텀이 있어. 그럴때 post-processing이 필요한데 그나마 최신 기술 NVDS가 속도과 정확도 측면에서 많이 부족하다. 그걸 우리가 개선해주겠다고 겸손하게 접근 필요 (나머지 장점들은 그냥 덤덤하게 실험에서 풀고 결론에 덧붙이지 뭐)}

%중요한 연구 배경
Video depth estimation, the task of inferring 3D scene structure from 2D video sequences, is important % as a cornerstone technology 
for a variety of modern applications such as autonomous driving, robotics, and mixed reality. Driven by this critical need, monolithic end-to-end~\yr{(E2E)} models, such as Video Depth Anything (VDA)~\cite{vda}, have established the current state-of-the-art, delivering exceptional coherence and spatial accuracy. 

However, \yr{the dominant E2E framework faces fundamental bottlenecks in practical deployment.} These models are typically designed as tightly coupled systems, leading to \yr{a significant adaptation lag.} % lag in the latest adaptation.
Whenever \yr{a superior} single image-to-depth estimator~\yr{(I2D)} is released, it cannot be easily integrated into existing \yr{E2E} frameworks without full-scale, \yr{computationally expensive} retraining. 
Moreover, these massive all-in-one systems are often \yr{memory-intensive for edge devices, creating a barrier to real-time deployment}.

\yr{To mitigate these issues,} modular post-processing methods like NVDS~\cite{nvds} \yr{have emerged as a promising} plug-and-play alternative.
\yr{By decoupling the video stabilization process from the image-level depth estimation, these methods allow for the immediate integration of evolving I2D models.
Despite their potential, however,} they have yet to match the efficiency of \yr{E2E} systems.
They often suffer from taking orders of magnitude long inference and reliance on RGB data, \yr{both of} which are critical bottlenecks for real-time applications.

In this work, we revitalize the role of post-processing in video depth estimation \yr{by demonstrating that it} can achieve not only competitive accuracy but also superior speed and scalability.
By moving away from monolithic architectures, our approach allows for the immediate integration of the \yr{evolving} I2D models into video streams.
% Furthermore, by avoiding computational overhead, our framework can be deployed on resource-constrained devices where memory is strictly limited. 
We propose a \yr{fundamental} shift in perspective: rather than reconstructing the full 3D world by analyzing complex color contexts in an RGB video---a process that makes existing post-processing models like NVDS~\cite{nvds, nvdsplus} computationally expensive---we argue for efficient geometric refining and restoring.
\yr{We observe that the per-frame depth maps already provide a fundamentally sound, albeit temporally unstable, 3D structure.}
% Our method starts with a simple assumption. The per-frame depth maps give us an unstable but already good 3D structure. 
This \yr{observation} reframes the task from a scene reconstruction problem into a more manageable structure correction problem.
\yr{Instead of rebuilding the 3D scene from color context, our approach focuses on rectifying}
% We do not need to rebuild the world from color. We only need to fix the 
unstable elements using geometric cues.
\yr{This design significantly reduces the computational barrier for deployment while establishing a scalable paradigm for geometry-only temporal stabilization.}
% Our work not only reduces the barrier for deploying rapid video depth in practical applications but also contributes a new, scalable paradigm for leveraging geometry-only information to ensure temporal stability.

As shown in Table~\ref{tab:comparison}, current video depth solutions involve trade-offs in practical deployment.
High-performance end-to-end models, such as VDA-L~\cite{vda}, establish a benchmark for temporal coherence but are often too computationally intensive for real-time edge use.
Although modular post-processing methods like NVDS~\cite{nvds} aim to bridge this gap, they struggle with high latency and reliance on RGB data, failing to reach the efficiency required for embedded applications.
In contrast, state-of-the-art single-image estimators such as DAv2~\cite{depthanythingv2} provide spatial accuracy and speed but lack the inherent temporal coherence for stable video streams.
%
\begin{table}[t]
\centering
\caption{\textbf{Comparison of video depth estimation paradigms.} VDPP provides a balanced profile for practical deployment, achieving SOTA-level coherence within a modular and efficient post-processing framework.}
\label{tab:comparison}
\small
\setlength{\tabcolsep}{5pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|l|ccccc}
\toprule
\textbf{Category} & \textbf{Method} & \textbf{Speed} & \textbf{Temporal} & \textbf{Plug \&} & \textbf{Depth} & \textbf{Light-} \\
 & & \textbf{($>30$ FPS)} & \textbf{Coherence} & \textbf{Play} & \textbf{Only} & \textbf{weight} \\
\midrule
\multirow{2}{*}{End-to-End} & VDA-S~\cite{vda} & \checkmark & $\triangle$ & $\times$ & $\times$ & $\times$ \\
 & VDA-L~\cite{vda} & $\times$ & \checkmark & $\times$ & $\times$ & $\times$ \\
\midrule
\multirow{2}{*}{Post-Processing} & NVDS~\cite{nvds} & $\times$ & $\times$ & \checkmark & $\times$ & $\times$ \\
% \rowcolor{green!15}
 & \textbf{VDPP (Ours)} & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
\bottomrule
\end{tabular}}
\raggedright
\footnotesize
* Lightweight capability is verified on the NVIDIA Jetson Orin Nano (8GB) without Out-of-Memory errors.
\vspace{-4mm}
\end{table}
%
%우린 이런 방법으로 설계했다.
\yr{In this paper, w}e propose \textbf{VDPP~(Video Depth Post-Processing)}, a framework that formulates video depth stabilization as a targeted geometric correction problem.
By precisely refining unstable per-frame depth sequences, VDPP addresses the efficiency and accuracy bottlenecks of previous post-processing methods.
This allows for robust coherence to real-time embedded applications without \yr{sacrificing} the flexibility of a modular architecture.
Figure~\ref{fig:teaser} provides a qualitative and quantitative overview of our results, including . % The left side displays the qualitative refinement achieved by VDPP, while the right side presents a quantitative comparison graph 
peformance benchmarks on the Sintel dataset~\cite{sintel} at a resolution of $384 \times 384$. The detailed numerical tables supporting this graph are provided in Appendix C.

\begin{itemize}
\item \textbf{Decoupled and Scalable Paradigm:} We propose an RGB-free, modular framework that \yr{resolves the adaptation lag of monolithic models, enabling the immediate integration of any evolving image-depth backbone or depth-only sensors such as LiDAR.} % revitalizes the role of post-processing. By eliminating the dependency on color context, we resolve the adaptation lag of monolithic models, enabling the immediate integration of any evolving image-depth backbone or depth-only sensors (e.g., LiDAR) into stable video streams.

\item \textbf{Embedded Efficiency and Real-time Deployment:} Designed for resource-constrained environments, \yr{VDPP achieves exceptional speed (>43.5 FPS) on an NVIDIA Jetson Orin Nano with a minimal memory footprint, ensuring viability for real-time edge applications.} % VDPP overcomes the latency bottlenecks of previous post-processing methods. We demonstrate that our framework achieves remarkable efficiency, reaching $> 43.5$ FPS on an NVIDIA Jetson Orin Nano with minimal memory footprint, making high-quality video depth viable for real-time edge applications.

\item \textbf{Geometric Refinement with Residual Learning:} We introduce a dual-component design (Depth + Normals) with downsampling and residual learning in error space. This technical shift focuses the network on targeted geometric correction rather than redundant scene reconstruction, allowing a lightweight architecture to match the temporal coherence of heavy end-to-end systems.
\end{itemize}


